Being-H0.5: Scaling Human-Centric Robot Learning for Cross-Embodiment Generalization

We introduce Being-H0.5, a foundational Vision-Language-Action (VLA) model designed for robust cross-embodiment generalization across diverse robotic platforms. While existing VLAs often struggle with morphological heterogeneity and data scarcity, we propose a human-centric learning paradigm that treats human interaction traces as a universal "mother tongue" for physical interaction. To support this, we present UniHand-2.0, the largest embodied pre-training recipe to date, comprising over 35,000 hours of multimodal data across 30 distinct robotic embodiments. Our approach introduces a Unified Action Space that maps heterogeneous robot controls into semantically aligned slots, enabling low-resource robots to bootstrap skills from human data and high-resource platforms. Built upon this human-centric foundation, we design a unified sequential modeling and multi-task pre-training paradigm to bridge human demonstrations and robotic execution. Architecturally, Being-H0.5 utilizes a Mixture-of-Transformers design featuring a novel Mixture-of-Flow (MoF) framework to decouple shared motor primitives from specialized embodiment-specific experts. Finally, to make cross-embodiment policies stable in the real world, we introduce Manifold-Preserving Gating for robustness under sensory shift and Universal Async Chunking to universalize chunked control across embodiments with different latency and control profiles. We empirically demonstrate that Being-H0.5 achieves state-of-the-art results on simulated benchmarks, such as LIBERO (98.9%) and RoboCasa (53.9%), while also exhibiting strong cross-embodiment capabilities on five robotic platforms.

==> table/human_data_list.tex <==
\begin{table*}[h!]
\centering
\caption{The robot data 
used for pretraining Being-H0.5 includes demonstrations from \textbf{29 distinct robotic embodiments} and encompasses over \textbf{11,000 hours}, resulting in \textbf{25.5 million} text token and \textbf{64.1 billion} image training tokens in total.
Episodes are labeled as ``grp'' (parallel gripper) or ``dex'' (dexterous hand), and as ``real'' (collected via real-world teleoperation) or ``sim'' (collected in simulation). The dataset features diverse camera views, varying robotic structures, and a wide range of scenarios.  
This collection represents the most diverse and largest robotic pretraining corpus to date. }
\setlength{\tabcolsep}{10pt}
\renewcommand{\arraystretch}{1.1}
\scalebox{0.9}{
    \begin{tabular}{l|c|c|c|c}
    \toprule
    \textbf{Robot Type} & \textbf{Camera Views} & \textbf{EEF Type} & \textbf{Data Source} & \textbf{Duration (Hours)} \\
    \midrule
    \textbf{Single-Arm Robots} & & & & \\
    \cmidrule(lr){1-1}
    Franka & ego, 3rd$\times$2, wrist & grp \& dex & real \& sim & 2196.4 \\
    Google Robot & ego, 3rd & grp & real \& sim & 597.5 \\
    Kuka-iiwa & ego, 3rd & grp & real \& sim & 169.11 \\
    WidowX & 3rd$\times$2, wrist & grp & real \& sim & 152.6 \\
    Xarm7 Robot & top, 3rd & grp & real \& sim & 297.24 \\
    UR5 & 3rd, wrist & grp & real \& sim & 104.14 \\
    Hello Stretch & ego, 3rd & grp & real & 135.14 \\
    Jaco & 3rd$\times$3 & grp & real \& sim & 97.22 \\
    Kinova3 & 3rd$\times$3 & grp & sim & 98.7 \\
    Sawyer & 3rd & grp & sim & 98.2 \\
    Cobotta & 3rd & grp & real & 5.3 \\
    DLR Sara & 3rd & grp & real & 6.06 \\
    PR2 & ego & grp & real & 5.97 \\
    \midrule
    
    \textbf{Dual-Arm Robots} & & & & \\
    \cmidrule(lr){1-1}
    RMC Aida L & high, wrist$\times$2 & grp & real & 162.87 \\
    Galaxea R1 Lite & high, wrist$\times$2 & grp & real & 630.56 \\
    Agilex Split ALOHA & high, wrist$\times$2 & grp & real \& sim & 1099.05 \\
    Agilex Cobot Magic & high, wrist$\times$2 & grp & real & 194.6 \\
    Piper & ego, wrist$\times$2 & grp & real \& sim & 904.54 \\
    \midrule
    
    \textbf{Portable Arm} & & & & \\
    \cmidrule(lr){1-1}
    BeingBeyond D1 & ego & dex & real & 100 \\
    SO101 & ego, wrist$\times$2 & grp & real & 97.22 \\
    \midrule
    
    \textbf{Half-Humanoid} & & & & \\
    \cmidrule(lr){1-1}
    PND Adam & ego & dex & real & 200 \\
    Agibot-G1 & \{ego, wrist\}$\times$2 & grp \& dex & real \& sim & 2391.67 \\
    Leju kuavo 4 LB & ego, wrist$\times$2 & grp \& dex & real & 1198.15\\
    AlphaBot 2 & ego, wrist$\times$2 & grp & real & 6.94 \\
    Airbot MMK2 & 3rd, wrist$\times$2 & grp & real & 11.55 \\
    Galbot G1 & wrist$\times$2 & grp & sim & 97.96 \\
    Tianqing A2 & high, wrist$\times$2 & grp & real & 9.75 \\
    \midrule
    
    \textbf{Humanoid} & & & & \\
    \cmidrule(lr){1-1}
    Unitree G1edu-u3 & ego, wrist$\times$2 & grp \& dex & real & 67.87 \\
    Tiankung & top & grp & real & 107.13 \\
    \midrule
    
    \textbf{Total: 29 embodiments} & & & & \textbf{11049.63} \\
    \bottomrule
    \end{tabular}
}
\label{tab:robot_data}
\end{table*}


==> table/real_robot_exps.tex <==
\begin{table}[h]
\centering
\caption{\textbf{Real-world success rates (\%) across heterogeneous platforms.} Each task is evaluated over 20 blind trials. Being-H0.5 consistently outperforms baselines across diverse embodiments, with the largest gains on bimanual coordination and few-shot adaptation scenarios.}
\label{tab:real_robot_main}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{ll|ccc >{\cellcolor{BlockA!30}}c}
\toprule
\textbf{Platform} & \textbf{Task} & \textbf{Scratch} & \textbf{$\pi_{0.5}$} & \textbf{Being-H0.5} & \textbf{Gain} \\
\midrule
\multirow{6}{*}{\shortstack[l]{\textbf{AdamU} \\ \scriptsize (31 DoF, Bimanual)}} 
    & Bimanual Pick-to-Box & -- & -- & \textbf{--} & -- \\
    & Bimanual Hand-Over   & -- & -- & \textbf{--} & -- \\
    & Pick-to-Drawer       & -- & -- & \textbf{--} & -- \\
    & Flower Arrangement   & -- & -- & \textbf{--} & -- \\
    & Liquid Pouring       & -- & -- & \textbf{--} & -- \\
    & Surface Wiping       & -- & -- & \textbf{--} & -- \\
\cmidrule{2-6}
    & \textit{Subtotal Average} & -- & -- & \textbf{--} & -- \\
\midrule
\multirow{5}{*}{\shortstack[l]{\textbf{Franka-Inspire} \\ \scriptsize (13 DoF, Tabletop)}} 
    & Multi-Bowl Stacking  & -- & -- & \textbf{--} & -- \\
    & Precise Placement    & -- & -- & \textbf{--} & -- \\
    & Block Stacking       & -- & -- & \textbf{--} & -- \\
    & Tool Use (Watering)  & -- & -- & \textbf{--} & -- \\
    & Surface Wiping       & -- & -- & \textbf{--} & -- \\
\cmidrule{2-6}
    & \textit{Subtotal Average} & -- & -- & \textbf{--} & -- \\
\midrule
\textbf{BeingBeyond D1} & Block Stacking & -- & -- & \textbf{--} & -- \\
\midrule
\textbf{Unitree G1} & Flip-and-Scan & -- & -- & \textbf{--} & -- \\
\midrule
\multicolumn{2}{l|}{\textbf{Overall Performance (Mean)}} & -- & -- & \textbf{\cellcolor{BlockA!30}--} & \textbf{+--\%} \\
\bottomrule
\end{tabular}
\end{table}



==> table/robot_platforms.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Detailed specifications of real robot platforms.} Being-H0.5 is validated across  diverse embodiments with varying DoF, control frequencies, and camera configurations.}
\label{tab:real_robot_platforms}
\setlength{\tabcolsep}{10pt} 
\small
\begin{tabular}{lcccccc}
\toprule
& & \multicolumn{3}{c}{\textbf{Degrees of Freedom (DoF)}} & & \\ \cline{3-5}
\textbf{Platform} & \textbf{Type} & \textbf{Arm} & \textbf{Hand} & \textbf{Total} & \textbf{Cameras} & \textbf{Freq.} \\
\midrule
AdamU & Humanoid & 7$\times$2 + 5$^\dagger$ & 6$\times$2 & 31 & 2 $\times$ 256$^2$ & 20 Hz \\
Unitree G1 & Bimanual & 7$\times$2 & 6$\times$2 & 26 & 1 $\times$ 256$^2$ & 20 Hz \\
Franka-Inspire & Single-arm & 7 & 6 & 13 & 2 $\times$ 512$^2$ & 50 Hz \\
BeingBeyond D1 & Compact & 6 & 6 & 12 & 1 $\times$ 256$^2$ & 10 Hz \\
\bottomrule
\multicolumn{7}{l}{\footnotesize $^\dagger$ Includes 3-DoF waist and 2-DoF neck articulation.}
\end{tabular}
\end{table}

